Dynamic Enumeration of Similarity Joins

This paper considers enumerating answers to similarity-join queries under dynamic updates: Given two sets of $n$ points $A,B$ in $\mathbb{R}^d$, a metric $\phi(\cdot)$, and a distance threshold $r > 0$, report all pairs of points $(a, b) \in A \times B$ with $\phi(a,b) \le r$. Our goal is to store $A,B$ into a dynamic data structure that, whenever asked, can enumerate all result pairs with worst-case delay guarantee, i.e., the time between enumerating two consecutive pairs is bounded. Furthermore, the data structure can be efficiently updated when a point is inserted into or deleted from $A$ or $B$. We propose several efficient data structures for answering similarity-join queries in low dimension. For exact enumeration of similarity join, we present near-linear-size data structures for $\ell_1, \ell_\infty$ metrics with $\log^{O(1)} n$ update time and delay. We show that such a data structure is not feasible for the $\ell_2$ metric for $d \ge 4$. For approximate enumeration of similarity join, where the distance threshold is a soft constraint, we obtain a unified linear-size data structure for $\ell_p$ metric, with $\log^{O(1)} n$ delay and update time. In high dimensions, we present an efficient data structure with worst-case delay-guarantee using locality sensitive hashing (LSH).

==> appndxBBDtree.tex <==
\subsection{Approximate Similarity Join under $\ell_2$ metric}
\label{appendix:l2}

In this section, we use the \emph{BBD} tree to derive our new index. We start by introducing BBD trees.

\paragraph{BBD tree.}
A balanced box decomposition (or BBD for short) tree~\cite{arya2000approximate, arya1998optimal} is a variant of the \emph{quadtree}~\cite{har2011geometric, samet1989spatial}. A BBD tree $\T$ on a set $P$ of $n$ points in $\mathbb{R}^d$, is a balanced binary tree of size $O(n)$ and height $O(\log n)$ with $n$ leaves. It can be constructed in $O(n\log n)$ time.
Every box has a bounded aspect ratio and every $2d$ levels of descent in the tree, the size of the associated cells decreased by at least a factor of $1/2$, where the size of a cell is defined as the length of its longest side.
Each node is associated with a box in $\mathbb{R}^d$ or the set theoretic difference of two nested boxes $\square_v^O, \square_v^I$ (rectangular annulus) with $\square_v^I$ possibly being empty. Hence each box $v$ is associated with an annular region $\square_v=\square_v^O\setminus \square_v^I$.


Given a sphere $B$ of radius $1$, the BBD tree in \cite{arya2000approximate, arya1998optimal}
returns $O(\log n + \eps^{d-1})$ nodes
such that the union of their regions
completely covers $B\cap P$ and might cover some parts of $(1+\eps)B$.
Given $x\in \Re^d, r\geq 0, \eps>0$, the BBD tree $\T$ can be %used to answer an $\eps$-approximate neighborhood query:
    \begin{itemize}
        \item all points of $P$ within distance $r$ from $x$ will be returned;
        \item no point of $P$ farther than $(1+\epsilon)r$ from $x$ will be returned;
    \end{itemize}
Points that are at distance from $x$ between $r$ and $(1+\eps)r$ from $x$ may or may not be reported. The time complexity of such a query is $O(\log n + \eps^{1-d}+k)$, where $k$ is the output size. 

In~\cite{eppstein2005skip, mount2010dynamic}, the dynamic version of BBD tree was proposed, with $\O(1)$ time for maintenance under per update.



%Similarly, we first partition points in $A$ into $m = O(\log n)$ groups $A^{(1)}, A^{(2)}, \cdots, A^{(m)}$, and build a BBD tree $\T^{(i)}$ for points only in $A^{(i)}$. We also build a dynamic BBD tree $\T_B$ for points in $B$. For a node $u$ in $\T_B$, let $p(u)$ be the parent of $u$, and $\size(\square_u)$ be the largest side of the box $\square_u$. 

\paragraph{Index}
We build two dynamic BBD trees for points in $A, B$ as $\T_A, \T_B$ separately. 
The dynamic property of $\T_A$ will be maintained by applying the transformation described in Section~\ref{sec:prelim}. In particular, we partition the points in $A$ into $m=\log |A|$ groups $A^{(1)}, A^{(2)}, \ldots, A^{(m)}$ and construct $\log |A|$ static BBD trees $\T^{(i)}$, for each $i=1,2,\ldots, m$. The construction of $\T_B$ will use the standard techniques in~\cite{eppstein2005skip, mount2010dynamic}, which supports $\O(1)$ amortized update time. These two indexes uses $\O(n)$ space and can be built in $\O(n)$ time.



\paragraph{Tripartite graph representation.}
Next, we will show how to define a tripartite graph representation $G =(A \cup C \cup B, E_1 \cup E_2)$. For a node $u$ in $\T_A$, let $p(u)$ be the parent of $u$, $\square_u$ be the box associated with $u$ and $\size(\square_u)$ be the largest side of the box $\square_u$. Define 
%The variable $u_f$ will have the value $1$ if there exists any point in $\square_u\cap A_i$ whose nearest neighbor in $B$ has distance at most $r=1$ and it will have the value $0$ if every point in $\sqaure_u\cap A_i$ has its nearest neighbor in $B$ within distance at least $(1+\eps)^2+\sqrt{d}\eps$.
\[C =\{u\in \T_A \mid \size(\square_u)\leq \eps/\sqrt{d}< \size(\square_{p(u)})\},\] i.e., the set of nodes that have size smaller than $\eps/\sqrt{d}$ but their parents have size strictly greater than $\eps/\sqrt{d}$.
Notice that $C$ defines a grid on the point set $A$ with small enough cells.
The BBD tree is actually used in our case to efficiently derive the cells of $C$ that are contained in a query ball.
%Observe that exactly one node for each root-to-leaf path is included by $C$, since the size of node is decreasing along the path.
%Thus, $C$ is a partition of the set $A$ with ``small enough" boxes.

The high-level idea why we choose these nodes from $\T_A$ as $C$ can be explained as follows. When a new ball is inserted or deleted from $B$, we need to find all nodes in $C$ whose union cover the ball (because of the error $\eps$ of the BBD tree, their union can also contain areas out of the ball).
%Because of the error $\eps$ of the BBD tree, we consider a slightly larger ball to ensure that we do not miss any point that is contained in the ball.
The size of nodes in $C$ is small enough so that the area out of the ball covered will be bounded, and also big enough so that for any unit ball $b \in B$, the number of nodes in $C$ to cover $b$ is bounded.

Consider an arbitrary node $u \in C$. For any point $a \in A$, edge $(a,u) \in E_1$ exists if $a \in \square_u$. However, for any point $b \in B$, edge $(b,u)$ is not constructed in a deterministic way; instead, it obeys the following rules due to the approximation nature of range queries over BBD tree: if $\lVert x-b \rVert_2 \le (1+\eps)^2$ for some corner $x$ of $\square_u$, $(b,u)$ exists; if $\lVert x-b \rVert_2 > (1+\eps)^3$, $(b,u)$ does not exist; otherwise, $(b,u)$ may or may not exist. 
%\xiao{However, the representation can be always conceptual, and will be explicitly clear when the enumeration begins.}
%\stavros{Why $(1+\eps)^3$? Also, using the BBD tree we are never sure if we will always return true in the following case: assume we search for a ball of radius $r$ and the error is $\eps$. Assume there is not point in the ball of radius $r$ but there is a point in the ball of radius $(1+\eps)r$. Then BBD tree might return true or false, so we cannot say for sure that we have an edge if this happens... We need to say it with two sentences or we need to define something to say what exactly going on here.}
%
%\stavros{Also, tbh I am not sure that the framework makes the discussion easier among all indexes. Like here it is not clear what is the construction time if we do not say how exactly we execute the queries. In an case professors can decide if we will keep the framework, I am just saying that I am not completely sure if it makes the discussion simpler or more vague.}
%%For each node $v\in C^i$ we also store $P_v=\{a \mid a\in \square_v \cap A_i\}$ in $v$.

\paragraph{Preprocessing.} Let $\mathcal{Q}_\eps(x,1+\eps)$ be an approximate range query on a BBD tree, where the query range is a ball of center $x$ and radius $1+\eps$, and the error parameter is $\eps$. We assume that $\mathcal{Q}_\eps(x,1+\eps)$ returns the set of nodes of the BBD tree whose union cover the ball $\mathcal{B}(x,1+\eps)$. 
%Such a query returns a set of nodes of a BBD tree whose union 

We define the inactive/active status of nodes in $C$. Node $u \in C$ is {\em active} if $\square_u \cap A\neq \emptyset$, and there exists a corner $x$ of $\square_u$ such that running the query $\mathcal{Q}_\eps(x, 1+\eps)$
in $\T_B$ it returns at least one point from $B$,
and {\em inactive} otherwise.
Notice that if a node $u\in C$ is active then $\square_u$ contains at least a point in $A$ and there exists at least one corner $x$ of $\square_u$ and a point $b\in B$ with $\lVert x-b\rVert_2\leq (1+\eps)^2$.
All active nodes are maintained in $\C$.
%
%
%For each $u \in C$, we introduce an indicator variable $u_\textrm{bool}$. %Let $v$ be a node in $C^i$ and let $C_v$ be the corners defined by the outer rectangle of node $v$. From the definition $|C_v|=O(1)$. For each point $x\in C_v$, let $\mathcal{B}(x, 1+\eps)$ be a sphere with center $x$ and radius $1+\eps$. 
%For any $u \in C$, if $\square_u \cap A\neq \emptyset$, and there exists a corner $x$ of $\square_u$ such that $\mathcal{B}_\eps(x, 1+\eps) \neq \emptyset$, then $u$ is {\active}; otherwise, $u_\textrm{bool} = 0$. 
%

%The proof of Lemma~\ref{lem:bbd-active} is given in Appendix~\ref{appendix:l2}. %%\stavros{Again, similarly to the previous case, we cannot say exactly that in plain language. We can say that if there exists a point from $B$ within distance $(1+\eps)$ then $v_\textrm{bool}=1$ and if there is no point within distance $(1+\eps)^2$ then it will be $v_\textrm{bool}=0$.}\xiao{"if there is no point within distance $(1+\eps)^2$ then it will be $v_\textrm{bool}=0$." and "if $v_\textrm{bool} = 1$, there exists a point from $B$ near one corner of $\square_v$, within distance $(1+\eps)^2$." seem equivalent to me.}


%\xiao{I didn't store points in $\square_u \cap A$ with $u$. Could these points be enumeratede with bounded delay?}

%%We approximate $\mathcal{B}(x, 1+\eps)$ by running a range query on $T_B$. The query returns true if there exists a point $b\in B$ such that $\lVert x-b\rVert_2 s\leq 1+\eps$ and false if for every $b\in B$, $\lVert x-b\rVert_2> (1+\eps)^2$. If the nearest neighbor of $x$ in $B$ has distance between $1+\eps$ and $(1+\eps)^2$, it might return true or false.
%
%We introduce a boolean indicator variable $v_\textrm{bool}$ for each node $v \in \T$. If there exists a corner $x \in \square_v$ such that $\mathcal{B}(x, 1, 1+\eps) \neq \emptyset$,  $v_\textrm{bool} = 1$; otherwise, $v_\textrm{bool} =0$. In plain language, if $v_\textrm{bool} = 1$, there exists a point from $B$ near $\square_v$.
%
%If the answer for at least one $x\in C_v$ is true, we set $v_f=1$, and $v_f = 0$ otherwise. In other words, if $v_f=1$ we are sure that there exists a point $b\in B$ which is close to the rectangle $\square_v$.
%
%In the end, we update $w_f$ for all nodes $w$ lying on the path from $v$ to the root of $T_i$ as follows. Let $w^1, w^2$ be the two children of $w$. If $w^1_f=1$ or $w^2_f=1$, we set $w_f=1$, and $w_f=0$ otherwise.

\begin{lemma}
\label{lem:bbd-active}
For any node $u \in C$, 
if $u$ is active, for any point $a \in A \cap \square_u$, there exists a point $b \in B$ such that $\lVert a-b\rVert_2\leq (1+\eps)^2 +\eps$; otherwise, there exists no pair of points $(a\in \square_v \cap A, b \in B)$ such that $\lVert a-b\rVert_2 \leq 1$. 
\end{lemma}
\begin{proof}
If $v$ is active, there exists a corner $x$ of $\square_v$ such that $\mathcal{Q}_\eps(x, 1+\eps)\neq \emptyset$. Let $b \in \mathcal{Q}_\eps(x, 1+\eps)$ be an arbitrary point. Moreover, $\lVert x-b\rVert_2 \le (1+\eps)^2$. As $\size(\square_v) \le \eps/\sqrt{d}$, the distance between any pair of points inside $\square_v$ is at most $\epsilon$. Then, for any point $a \in \square_v \cap A^{(i)}$, $\lVert a-b\rVert_2 \le \lVert x-b\rVert_2 + \lVert x-a\rVert_2 \le (1+\eps)^2 + \eps$. 

If $v$ is inactive, assume there is a pair of points $a\in \square_v\cap A_i, b\in B$ with $\lVert a-b\rVert_2 \leq 1$. As $\size(\square_v)\leq \eps/\sqrt{d}$, any pair of points in $\square_v$ has its distance bounded by $\epsilon$. Let $x$ be an arbitrary corner of $\square_v$. We will have  $\lVert x-b\rVert_2 \le \lVert a-b\rVert_2  + \lVert x-a\rVert_2 \leq 1+\eps$, contradicting the fact that $v$ is inactive, i.e., no corner of $\square_v$ has a near neighbor in $B$ within distance $1+\eps$.
\end{proof}



%The dynamic BBD tree $\T_B$ can be constructed in $O(n\log n)$ time using \cite{eppstein2005skip, mount2010dynamic}. Each static BBD tree $\T$ can be constructed in $O(2^i\log 2^i +2^i\eps^{1-d}\log n)$ time. 
%Moreover, the status in the tripartite graph $G$ can be constructed in $O(n\eps^{1-d}\log n)$ time, since each node in $C$ can be checked in $O(\eps^{1-d}\log n)$ time.
Note that the status of $u$ can be decided in $O(\eps^{1-d} \log n)$ time, so this step takes $O(n \eps^{1-d}\log n)$ time in total.
%The space of our index is $O(n)$.

\subsubsection{Update}
Note that the dynamic BBD tree $\T_B$ can be updated in $O(\log n)$ time, following the standard techniques in~\cite{eppstein2005skip, mount2010dynamic}.  Next, we focus on the update on $\T$ and $G$.

In the first case when an update happens for points in $A$, say $a$, we follow the standard techniques in \cite{bentley1980decomposable, erickson2011static}.

\paragraph{Insertion of $a$.}
Let $i$ be the smallest index such that $A^{(i)} =\emptyset$. We delete all BBD trees for every group $j \leq i$ and create a new BBD tree $\T^{(i)}$ on points in $\{a\} \cup (\bigcup_{j\leq i} A_j)$. Following the observations in \cite{bentley1980decomposable, erickson2011static},
 %if charging $O\left(\frac{1}{n} \cdot n\eps^{1-d}\log n\right)$ for each insertion,
the amortized cost is  $O(\eps^{1-d}\log n)$.

\paragraph{Deletion of $a$.}
Assume $a \in A^{(i)}$. Let $u$ be the leaf node in $\T^{(i)}$ containing $a$. We just remove $a$ from $u$. Let $v \in C$ be the node lying on the path from root to $u$. If $v$ is active and $\square_v \cap A^{(i)} = \emptyset$, i.e., there is no other point lying inside $\square_u$ except $a$, we remove $v$ from $\C$. %leaf that contains $a$ in $O(\log n)$ time. Then we delete $a$ from the leaf and then we visit each node $u$ from leaf to the the root of $T_i$. When reaching a node $v\in C^i$ we remove $a$ from $P_v$. If $P_v=\emptyset$, set $v_f=0$ and we update (if needed) all $u_f$ variables for nodes $u$ from $v$ to the root of $T_i$. 
Note that $\T^{(i)}$ is static, so no operations are performed on the tree structure. %It also follows from standard techniques in \cite{bentley1980decomposable, erickson2011static} (look 1.4 in \cite{erickson2011static}). We update $D=D+1$ (the number of deleted items is increased by $1$). Let $i$ be the group such that $a\in A_i$. By searching over tree $T_i$ we find the leaf that contains $a$ in $O(\log n)$ time. Then we delete $a$ from the leaf and then we visit each node $u$ from leaf to the the root of $T_i$. When reaching a node $v\in C^i$ we remove $a$ from $P_v$. If $P_v=\emptyset$, set $v_f=0$ and we update (if needed) all $u_f$ variables for nodes $u$ from $v$ to the root of $T_i$.

When the number of deleted points in $A$ is more than the number of the remaining points in $A$,
we just stop updating the existing index and build the set of $O(\lceil \log |A| \rceil)$ static BBD trees from scratch. Note that this index can be constructed in $O(n \cdot \eps^{1-d}\log n)$ time, the amortized cost is $O(\eps^{1-d}\log n)$.

\medskip
In the second case when an update comes from $B$, say $b$, we perform the following procedure for each group $A^{(i)}$ if $A^{(i)} \neq \emptyset$.
The high-level idea is to find all nodes in $C$ whose status would be changed by $b$, and update them if necessary. Let $U$ be the set of nodes returned by issuing a range query $\mathcal{Q}_\eps(b,(1+\eps)^2)$ to $\T^{(i)}$. The following Lemma states that every node in $U$ is located ``above'' the nodes in $C$.

\begin{lemma}
\label{lem:above}
For each $u\in U$, $size(\square_{p(u)})\geq \eps/\sqrt{d}$.
\end{lemma}
\begin{proof}
Let $v\in C$ be a node visited by the search procedure $\mathcal{Q}_\eps(b, (1+\eps)^2)$ in $\T^{(i)}$. We argue that the search algorithm will not continue searching at the children of $v$. 
The search procedure in \cite{arya2000approximate, arya1998optimal} first checks if $\square_v\subset \mathcal{B}(b, (1+\eps)^3)$. If that is true then the search procedure does not consider the children of $v$ and $v\in U$. If $\square_v\not\subset \mathcal{B}(b, (1+\eps)^3)$ then it checks if $\square_v\cap \mathcal{B}(b, (1+\eps)^2) = \emptyset$. If it is true then it does not consider the children of $v$ and $v\notin U$. Hence, the only remaining case to consider is when $\square_v\not\subset \mathcal{B}(b, (1+\eps)^3)$ and $\square_v\cap \mathcal{B}(b, (1+\eps)^2) \neq \emptyset$. However, this case will not happen because $\size(\square_v)\leq \eps/\sqrt{d}$: if $\square_v\not\subset \mathcal{B}(b, (1+\eps)^3)$ then $\square_v$ is so small that it does not intersect $\mathcal{B}(b, (1+\eps)^2)$. In particular, any pair of points in $\square_v$ has distance at most $\eps$ and the distance of $\mathcal{B}(b, (1+\eps)^2)$ and $\mathcal{B}(b, (1+\eps)^3)$ is more than $\eps$, so if $\square_v\not\subset \mathcal{B}(b, (1+\eps)^3)$ then $\square_v\cap \mathcal{B}(b, (1+\eps)^2) = \emptyset$.
\end{proof}




For each $u\in U$, we find all nodes in $C$ which reside in the subtree of $\T^{(i)}$ rooted at $u$, denoted as $V_u$. Note that we will check the status for each node $v \in \bigcup_{u \in U} V_u$. To see why this procedure is correct, it suffices to show that every node of $C$ whose status will be changed by the update of $b$ must be included by $\bigcup_{u \in U} V_u$.
In particular, it suffices to show that when a point $b$ is deleted from $B$, we will visit all nodes $u\in C$ such that there exists some corner $x$ of $\square_u$ with $\lVert x-b\rVert_2\leq (1+\eps)^2$. Let $u$ be such a node in $C$. Notice that $\square_u\cap \mathcal{B}(b, (1+\eps)^2)\neq \emptyset$. As $\size(\square_u) \le \eps/\sqrt{d}$, we observe that $\square_u \subset \mathcal{B}(b, (1+\eps)^3)$. Hence the search procedure for the query range $\mathcal{Q}_\eps(b, (1+\eps)^2)$ in $\T^{(i)}$ will always find a node $w$ that lies in the path from the root to $u$ such that $\square_w\subseteq \mathcal{B}(b, (1+\eps)^3)$. Notice that $\square_u\subseteq \square_w$. Hence, the search procedure always visits node $u$.

\paragraph{Insertion of $b$.} If $\square_v \cap A^{(i)} \neq \emptyset$ and $v$ is inactive, we compute the distances between all corners of $\square_v$ with $b$. If any one of them has distance smaller than $1+\eps$ from $b$, we add $v$ to $\C$.

%\remove{if any of its corners in $C_v$ has a nearest neighbor in $B$ within distance $1+\eps$ (it might return true even if the nearest neighbor is within distance $(1+\eps)^2$). This is similar to the procedure we consider in the preprocessing phase. If this is true (and $P_v\neq \emptyset$) then we set $v_f=1$. Otherwise we set $v_f=0$.}
%In the end we update (if needed) all variables $w_f$ from $\bigcup_{u\in U} V_u$ to the root of $T_i$.

\paragraph{Deletion of $b$.}
If $v$ is active and $\square_v \cap A^{(i)} \neq \emptyset$, we issue a range query $\mathcal{Q}_\eps(x, 1+\eps)$ to $\T_B$ for every corner $x$ of $\square_v$. If all queries have empty results, we remove $v$ from $\C$. %there is any other point The deletion of a point $b\in B$ is almost similar to to the insertion of the point. The only difference is that when we visit the nodes in $v\in V_u$ for $u\in U$, we need to run an approximate range query on $T_B$ to decide if there exists any $x$ of $\square_v$ and $b'\in B - \{b\}$ such that $\lVert x- b' \rVert_2 \leq 1+\eps$.

\medskip We next analyze the complexity of this update procedure with $b$. A first observation on the number of nodes we have checked is stated in Lemma~\ref{lem:numnodes}.

\begin{lemma}
\label{lem:numnodes}
$|\bigcup_{u\in U} V_u|=O\left(\eps^{-2d}(\log 2^i + \eps^{1-d})\right)$.
\end{lemma}
\begin{proof}
From \cite{arya2000approximate, arya1998optimal}, $|U|=O(\log 2^i +\eps^{1-d})$. From each node $u\in U$ we need to bound $|V_u|$. Notice that $size(\square_u)\leq 2(1+\eps)^3$.
Recall, that every $2d$ levels of the BBD tree $\T^{(i)}$ the size of the cells are decreased by at least a factor of $1/2$.
Hence, $2d\log(\frac{2(1+\eps)^3\sqrt{d}}{\eps})$ levels below the level of $u$ the size of the cells will be at most $\eps/\sqrt{d}$.
So, $|V_u|=O\left(2^{2d\log(\frac{2(1+\eps)^3\sqrt{d}}{\eps})}\right)=O\left((\frac{2(1+\eps)^3\sqrt{d}}{\eps})^{2d}\right)$.
\end{proof}

%\begin{lemma}
%\label{lem:bbd-update}
%The update time is $O(\eps^{1-3d} \log^2 n (\log n+\eps^{1-d}))$ if a point is inserted to or deleted from $B$.
%\end{lemma}
%rFirst, a point can be inserted (or deleted) in $\T_B$ in $O(\log n)$ time \cite{eppstein2005skip, mount2010dynamic}.
The range query over $\T^{(i)}$ takes $O(\log 2^i + \eps^{1-d})$ time, following~\cite{arya2000approximate, arya1998optimal}. Over all groups, it takes $O(\log n(\log n+\eps^{1-d}))$ to find all nodes in $U$. 
From Lemma~\ref{lem:numnodes} the insertion time is
$O(\eps^{-2d}\log n(\log n+\eps^{1-d}))$. Moreover, each range query over $\T_B$ takes $O(\eps^{1-d}\log n)$ time. Implied by the Lemma~\ref{lem:numnodes} we will execute $O(\eps^{-2d}\log n(\log n+\eps^{1-d}))$ such queries when we delete a point in $B$ so the overall update time for deleting a point is $O(\eps^{1-3d}\log^2 n(\log n+\eps^{1-d}))$.





%Next we show the analysis of the algorithm above.
%The next lemma shows that our search algorithm will never visit nodes whose corresponding cells have size smaller than $\eps/\sqrt{d}$. As a result, we will always be able to find nodes in $V_\eps^i$ running a BFS.


%\begin{lemma}
%\label{lem:visitAll}
%Our algorithm visits all nodes $u\in C^i$ such that there exists some point $x\in C_u$ with $\distEucl{x}{b}\leq (1+\eps)^2$.
%\end{lemma}
%\begin{proof}
%Let $v$ be a node in $C^i$ such that there exists $x\in C_v$ with $\distEucl{x}{b}\leq (1+\eps)^2$. Since $\square_v\cap B_S\neq \emptyset$ it also holds that $\square_v\subset B_S'$. Hence, the search procedure of the BBD tree will always find a node $w\in U$ that lies in the path from the root to $v$ such that $\square_w\subset B_S'$.
%Notice that $\square_v\subseteq \square_w$. Hence, the algorithm will visit the node $v$ starting a BFS from node $w$.
%\end{proof}


\subsubsection{Enumeration}
We visit each group $A^{(i)}$ if $A^{(i)} \neq \emptyset$. For any node $u \in \C$, we invoke the following procedure.
For each point $a \in A^{(i)} \cap \square_u$, let $B_a$ be the result of issuing a ball query $\mathcal{Q}_\eps(a, (1+\eps)^3)$ to $\T_B$. We just report $(a,b)$ for all $b$ in $B_a$.

%For each point $a \in A^{(i)} \cap \square_u$, let $B_u$ be the result of issuing sphere queries $\mathcal{B}_\eps(x, (1+\eps)^2)$ to $\T_B$, for every corner $x$ of $\square_u$. We just report all pairs $(a,b)$ in the cross product of $(A^{(i)} \cap \square_u) \times B_u$.

Each range reporting query over $\T_B$ takes $O(\eps^{1-d}\log n)$ time first, and then all results can be reported with  $O(1)$ delay. The delay of this enumeration phase is $O(\eps^{1-d}\log n)$.



%\xiao{can we just issue the queries $\mathcal{B}_\eps(x, (1+\eps)^2)$ for each corner $x$ of $\square_u$?}

%We start an inorder traversal of the tree $T_i$ accessing only the nodes $u$ with $u_f=1$. When the inorder traversal visits a node $u\in C^i$ with $u_f=1$ then we do the following: For each point $a \in p(u)$, we search $T_B$ with the sphere $\mathcal{B}(a, (1+\eps)^3)$. For any point $b$ reported from $T_B$, we enumerate the pair $(a, b)$.

%\begin{lemma}
%\label{lem:visitExist}
%When the algorithm visits a node $u\in C^i$ with $u_f=1$, then there exists at least a pair of points $(a\in \square_u\cap A_i, b\in B)$ such that $\distEucl{a}{b}\leq (1+\eps)^2+\eps$.
%\end{lemma}
%\begin{proof}
%Since $u_f=1$, we have that there is at least a point $b\in B$ such that $\distEucl{x}{b}\leq (1+\eps)^2$ for an $x\in C_u$. Furthermore, $\square_u\cap A_i\neq \emptyset$ (otherwise $u_f=0$) and the largest distance in $\square_u$ is $\eps$, so there will be a point $a\in \square_u\cap A_i$ such that $\distEucl{a}{b}\leq (1+\eps)^2+\eps$.
%
%In order to complete the proof we need to make sure that if $b\in B$ is the only point in $B$ which is ``close" to the $\square_u$ and we delete $b$ then we will indeed update $u_f$ to be $0$ and not $1$. In other words, we need to ensure that when we delete $b$ we will visit the node $u$. This follows from Lemma~\ref{lem:visitAll}.
%\end{proof}

\begin{lemma}
\label{lem:bbd-approximate}
The index supports $(4\eps+6\eps^2+4\eps^3 + \eps^4)$-approximate enumeration.
\end{lemma}
\begin{proof}
It suffices to show that all pairs of points within distance $r$ must be reported, and any pair of points within distance strictly larger than $(1+\eps)^4$ will not be reported. 

Consider an arbitrary pair of points $(a, b) \in A \times B$ with $\lVert a-b \rVert_2 \leq 1$. Let $u \in C_\eps^i$ be the unique node such that $a \in \square_u$.
Observe that there exists a corner $x$ of $\square_u$ such that $\lVert x-b \rVert_2 \le  \lVert a-b \rVert_2 + \lVert x-a \rVert_2  \leq 1+\eps$, thus $u$ is active. So the enumeration query will visit node $u$ and we will run a query $\mathcal{Q}_\eps(a,(1+\eps)^3)$ in $\T_B$ finding the point $b$. When $u$ is active, for a node $u\in C$ then we will always return at least a pair $(a\in \square_u, b\in B)$ since there exists $b$ with $\lVert x-b\rVert_2\leq (1+\eps)^2$, where $x$ is a corner of $\square_u$ and $\lVert a-b\rVert_2\leq (1+\eps)^2+\eps<(1+\eps)^3$.

Finally, from the definition, a reporting query $\mathcal{Q}_\eps(a,(1+\eps)^3)$ in $\T_B$ will never return a point $b$ with $\lVert a-b\rVert_2>(1+\eps)^4$.
%While $b$ exists in $B$ we will always have $u_f=1$ (follows from Lemma~\ref{lem:visitAll} and the construction of the index $L$).
%
%
%
%Next, consider any pair of points $(a,b) \in A \times B$ with $\lVert a - b \rVert_2 \ge (1+\eps)^4$. Assume it is reported. Then, $a \in A^{(i)} \cap \square_u$, and there must exist a corner $x$ of $\square_u$ such that $b$ is returned by the sphere query $\mathcal{B}_\eps(x, (1+\eps)^2)$. In this way, we can bound $\lVert a-b \rVert_2 \le \lVert a-x \rVert_2 + \lVert x-b \rVert_2 \le \eps + (1+\eps)^3 < (1+\eps)^4$, coming to a contradiction.
%
%Next, for any pair of points $(a, b)$ reported, $b$ is found by the a sphere query $\mathcal{B}_\eps(a, (1+\eps)^3)$ to $\T_B$. By the definition of approximated sphere query, only points within distance $(1+\eps)^4$ from $a$ will be returned, thus $\lVert a-b\rVert_2 \le (1+\eps)^4$.
%
%
%From the previous Lemma~\ref{lem:visitExist} we have that when the enumeration algorithm visits $u\in C_\eps^i$ with $u_f=1$ will it always reports a pair $(a\in \square_u\cap A_i, b\in B)$ since $(1+\eps)^3> (1+\eps)^2+\eps$. When we run the search procedure in $T_B$ with the query range $\mathcal{B}(a, (1+\eps)^3)$ %
%
%
%it might also return a point $b\in B$ within distance $(1+\eps)^4$ from $a$ \cite{eppstein2005skip, mount2010dynamic}.
%Hence we conclude that our algorithm might return pairs $(a, b)$ with $\distEucl{a}{b}\leq (1+\eps)^4$.
\end{proof}

%By setting $\eps' = \frac{\eps}{6}$, the complexity remains the same asymptotically, as long as $d$ is a constant. The approximation ratio can then be simplified as $(1+\frac{\eps}{6})^4 \le 1+\eps$. Together, we conclude to the following theorem. 

==> conclusion.tex <==
\section{Conclusion}

In this paper, we consider how to use indexes for enumerating answers to similarity join queries; these indexes also support data updates. We present several efficient indexes for similarity join under $\ell_1$, $\ell_2$, and $\ell_\infty$ metrics (some of our results can be extended to other metrics). 

Note that our indexes provide worst-case delay guarantee for arbitrary updates and arbitrary input data. In practice, most real-world update sequences are ``nice'', nowhere near these worst-case scenarios; and input points from two sets are always dependent, or follow certain parameterized distributions. A more fine-grained analysis on the intrinsic difficulty of dynamic enumeration over similarity joins is interesting but still open. Similar instance-dependent analysis has been considered in~\cite{wang2020maintaining}.

The next interesting question is to consider other variants of similarity join queries under more general metrics, for example with constant doubling dimension, and distance functions, for example the cosine function used for measuring the similarity if the input vectors are sparse. 

%For example, it might be possible that some of our techniques in this paper can be extended to metrics with constant doubling dimension. Furthermore, we would like to consider the problem of dynamic enumeration of similarity join under more general similarity functions, not necessarily metrics. For instance, due to its low-complexity for sparse vectors, some applications use the cosine distance to measure the similarity of two points/vectors. An interesting open problem to consider is the dynamic enumeration of similarity joins under the cosine distance.

==> framework.tex <==
\section{Framework}
\label{sec:framework}
\newcommand{\graph}{G'}
\newcommand{\setCliques}{\mathcal{F}}
All our algorithms for solving similarity join in different settings are based on a common framework.  Intuitively, we model the similarity join as a bipartite graph $\graph = (A\cup B, E)$, where an edge $(a,b) \in E$ exists if and only if $a$ can be joined with $b$, i.e., $\dist(a,b) \le r$. To obtain a data structure for poly-logarithmic delay enumeration, it suffices to find a compact representation of $\graph$ with a set $\setCliques=\{(A_1, B_1), (A_2, B_2),\ldots, (A_u,B_u)\}$ of edge-disjoint bi-cliques such that (i) $A_i\subseteq A$, $B_i\subseteq B$ for any $i$, (ii) $E = \bigcup_{i=1}^u A_i \times B_i$, and (iii) $(A_i \times B_i) \cap (A_j \times B_j) = \emptyset$ for any $i \neq j$.
It remains to store and maintain these bi-cliques efficiently under update.

Take equi-join as an example. After representing input tuples as sets of vertices $A$ and $B$, there is an edge between $a \in A$ and $b \in B$ if and only if $a$ and $b$ have the same join attribute value. In this way, the bipartite graph itself is a set of edge-disjoint bi-cliques. However, this bipartite representation is not resilient to update, i.e., an insertion or deletion of any tuple may incur $\Omega(n)$ changes in the worst case. A simple idea of getting around this problem is to introduce a middle layer of vertices as $C$, each representing a distinct join attribute value and there is an edge between $a \in A$ (resp. $b \in B$) and $c \in C$ if and only if the join attribute value of $a$ (resp. $b$) is equal to $c$. An example is illustrated in Figure~\ref{fig:equi-join}. 
\begin{figure}
    \centering
    \includegraphics[scale = 0.8]{equi-join}
    \caption{An example of equi-join $R_1(X,C) \Join R_2(C,Y)$.}
    \label{fig:equi-join}
\end{figure}

Let $A_c \subseteq A, B_c \subseteq B$ be the set of vertices in $A,B$ with join attribute value $c$. In our construction, $A_c, B_c$ are exactly the list of vertices which share an edge with $c$, thus the biclique $A_c \times B_c \subseteq E$ is implicitly represented by the cross product of two neighbor lists of $c$. To achieve constant-delay enumeration, we need to maintain a list of {\em active} values in $C$, i.e., $c \in C$ is active if and only if $c$ is connected to at least one 
value in $A$ and one value in $B$. Obviously, we only visit active values in $C$, each emitting at least one result. This improves the original representation in the following way: (1) it decreases the space complexity as well as the pre-processing time complexity from $O(n+k)$ to $O(n)$, where $k$ is the output size; (2) the update time is decreased from $O(n)$ to $O(1)$.  


We extend this simple example to general similarity joins with $r > 0$. A formal description of the framework is defined as follows.

\begin{definition}[Tripartite Graph Representation]
A tripartite graph $G = (A \cup C \cup B, E_1 \cup E_2)$ where $E_1 \subseteq A \times C$ and $E_2 \subseteq C \times B$ is a representation of the similarity join over $A, B$ under $\dist(\cdot)$ metric with threshold $r$ if for each pair of points $(a, b) \in A \times B$ with $\dist(a,b) \le r$, there exists unique $c \in C$ such that $(a,c) \in E_1, (c, b) \in E_2$.
\end{definition}

It should be noted that $G$ is only conceptual, instead of being stored explicitly. The only extra information we will maintain for $G$ is the {\em status} of vertices in $C$. Let $A_c, B_c$ be the set of vertices in $A, B$ connected to $c \in C$, respectively. To support constant-delay enumeration, we define a vertex $c \in C$ as {\em active} if it witnesses at least one result, i.e., $A_c \neq \emptyset$ and $B_c \neq \emptyset$, and {\em inactive} otherwise. All active vertices are maintained in $\C \subseteq C$. 

\begin{lemma}[$\delta$-delay Enumeration]
\label{lem:fw-enumerate}
In $G = (A \cup C \cup B, E_1 \cup E_2)$ with a set of active vertices in $C$ as $\bm{\mathcal{C}}$, if for any $c \in C$, vertices in $A_c$ (resp. $B_c$) can be enumerated with $\delta$ delay, then all join results can be enumerated with $\delta$ delay.
%\begin{itemize}
%    \item whether $A_c = \emptyset$ (or $B_c = \emptyset$) can be decided in $\delta$ time; and
%    \item vertices in $A_c$ (resp. $B_c$) can be enumerated with $\delta$ delay;
%\end{itemize}
%then all join results can be enumerated with $\delta$ delay.
\end{lemma}

The proof of Lemma~\ref{lem:fw-enumerate} directly follows the algorithm: We visit each vertex $c \in \C$, and enumerate every pair $(a,b)\in A_c \times B_c$ by a nested-loop over $A_c, B_c$. It remains to show how to compute and update the active/inactive status of vertices $C$. The proof of Lemma~\ref{lem:status} is given in Appendix~\ref{appendix:framework}.

\begin{lemma}[Status Maintenance]
\label{lem:status}
In $G = (A \cup C \cup B, E_1 \cup E_2)$ with $|C| = O(\eta)$, if (1) for any $c \in C$, whether $A_c = \emptyset$ and $B_c = \emptyset$ can be decided in $\delta$ time; (2) for any $c \in C$, $A_c$ and $B_c$ can be counted in $\zeta$ time; (3) for any $a \in A$ (reps. $b \in B$), $C_a$ (or $C_b$) can be reported in $\lambda$ time, then we have two possible options for $\C$ as below: 
\begin{itemize}
    \item $\C$ can be computed in $O(\eta \delta)$ time and updated in $O(\lambda \delta)$ time; 
    \item $\C$ can be computed in $O(\eta \zeta)$ time and updated in $O(\lambda)$ time. 
\end{itemize}
%\begin{itemize}
%    \item $|C| = O(\eta)$;
%    \item for any $c \in C$, the $A_c$ and $B_c$ can %be counted in $\zeta$ time;
%%%\end{itemize}
%then the status of vertices in $C$ can be computed in $O(\eta \cdot \lambda)$ time and updated in $O(\zeta)$ time.
\end{lemma}

%\begin{lemma}[Maintenance under Update]
%\label{lem:index}
%In $G = (A \cup C \cup B, E_1 \cup E_2) $, if $|C|= O(\eta)$ and for each $a \in A$ (resp. $b \in B$), $|C_a|= O(\zeta)$ (resp. $|C_b| = O(\zeta)$), then $G$ can be built in $O(\delta \cdot \min\{\eta, n \cdot \zeta\})$ time with $O(n \cdot \zeta)$ space, and updated in $O(\zeta \cdot \delta)$ time, where $\delta$ is the delay of enumeration in Lemma~\ref{lem:fw-enumerate}.
%\end{lemma}
%
%
%
%
%
%For each vertex $c \in C$, we only need $O(1)$-size space for storing its status and necessary information. Thus, the total space used for $G$ is $O(|C|) =O(\eta)$. Next, we show two easy algorithms for pre-processing and updating $G$.
%
%Note that in the pre-processing step, the only information to be stored for $G$ is the active/inactive status of vertices in $C$. Initially, for each vertex $c \in C$, we spend $2 \cdot \lambda$ time to compute $\mu_A(c) = |A_c|$ and $\mu_B(c) = |B_c|$, If $|A_c| > 0$ and $|B_c| > 0$, we add $c$ to $\C$.  In total, this step takes $O(\lambda \cdot |C|) = O(\lambda \cdot \zeta)$ time. 
%Let $|C|= O(\eta)$ and for each $a \in A$ (resp. $b \in B$), $|C_a|= O(\zeta)$ (resp. $|C_b| = O(\zeta)$). Next, we describe how to build and update $G$. % built in $O(\delta \cdot \min\{\eta, n \cdot \zeta\})$ time with $O(n \cdot \zeta)$ space, and updated in $O(\zeta \cdot \delta)$ time.
%
%Observe that each edge in $E_1 \cup E_2$ has one of its endpoint in $A \cup B$, thus $|E_1 \cup E_2| \le n \cdot (\max_{a \in A} |C_a| + \max_{b \in B} |C_b|)= O(n \cdot \zeta)$, which also implies $C = O(n \cdot \zeta)$. Note that in the pre-processing step, the only information to be stored for $G$ is the active/inactive status of vertices in $C$. Initially, for each vertex $c \in C$, we spend $2 \cdot \delta$ time to check whether $A_c = \emptyset$ and $B_c = \emptyset$, and distinguish it as active or inactive. In total, this step takes $O(\delta \cdot |C|) = O(\delta \cdot \min\{\eta, n \cdot \zeta\})$ time. 
%
%When an update occurs, say a point $a$ is inserted to $A$ (the case of deletion is similar), the high-level idea is to check if some vertex in $C_a$ turns active after the insertion of $a$. We first find $C_a$ by a reporting query. For each $c \in C_a$, we increase $\mu_A(c)$ by $1$. If $c \in \C$, we check whether $\mu_{B}(c) > 0$; if yes, add $c$ to $\C$. This step takes $O(|C_a|) = O(\lambda)$ time.  
%his step can be done in $O(\zeta)$ time. Moreover, we need to update the active/inactive status of vertices in $C$. In this case, some inactive vertices may turn into active after the insertion of $a$. For each vertices $c \in C_a$, if it is inactive, we check whether $B_c = \emptyset$. If $B_c \neq \emptyset$, we add $c$ to $\bm{\mathcal{C}}$.  By Lemma~\ref{lem:fw-enumerate}, each check can be done in $\delta$ time. As $|C_a|\le \zeta$, this step can be done in $O(\delta \cdot \zeta)$ time. The construction of $G$ can be simply done by inserting every point of $A \cup B$ to $G$, which takes $O(n \cdot \delta \cdot \zeta)$ times in total.

%We conclude to the next lemma.



In the remaining of this paper, we will see different instantiations of this framework. The details might be slightly different from what have been described here, due to the inherent difficulties of similarity joins in different settings. %by presenting a tripartite graph representation $G = (A \cup C \cup B, E_1 \cup E_2)$, such that
%\begin{enumerate}
%    \item For each $c \in C$, vertices in $A_c$ and $B_c$ can be enumerated with $O(\polylog{n})$ delay;
%    \item For each $a \in A$ (resp. $b \in B$), all vertices in $C_a$ (resp. $C_b$) can be reported in $O(\polylog{n})$ time.
%\end{enumerate}
%Implied by Lemma~\ref{lem:enumerate} and Lemma~\ref{lem:index}, $G$ is such a desired index that can be built in $O(n \polylog{n})$ pre-processing time with $O(n \polylog{n})$ space, updated in $O(\polylog{n})$ update time and support $O(\polylog{n})$-delay enumeration. 


==> lsh_new.tex <==
\clearpage
\newpage
====================================================
\section{thoughts}
\stavros{Here I just repeat the text we have in the lsh  but arguing that the number of conflicts of a point p is not $O(n^\rho)$, but it is $O(1)$. Again, that follows because the probability that $p, q$ have large distance and collide at the same bucket is $\beta^k=1/n$. For example check this presentation (slide 45) https://graphics.stanford.edu/courses/cs468-06-fall/Slides/aneesh-michael.pdf or even Sariel's book}
In general without this uniform assumption, we need to explore more properties of the LSH family for an efficient index. Our observation is that after checking some pairs of points in one bucket (the specific numbers of pairs will be determined later), we can safely skip the bucket, since with high probability any join result missed in this bucket will be found in another one. In this way, we avoid spending too much time in one bucket before finding any join result.

By choosing $k = O(\log n)$ and $\tau=O(n^{1/\rho})$, a nice property on this combination of parameters was proved for answering ANN query, which will be the starting point of our index.


\begin{lemma}[\cite{gionis1999similarity}]
\label{lem:nnq_2}
    For a set of $n$ points $P$ in hamming space $\mathbb{H}^d$ and a distance threshold $r$, by choosing $k=O(\log n)$, and $\tau=O(n^{\rho})$, the following two properties hold for every point $q \in P$:
\begin{itemize}
    \item Let $p$ be a point such that $\dist(p, q) \leq r$. With probability at least $3/4$, the point $q$ will collide in some bucket with point $p$;
    \item Let $P(q, (1+\epsilon)r)$ be the set of points in $P$ with distance more than $(1+ \epsilon)r$ from $q$. With probability at least $3/4$, the total number of distinct points in $P(q, (1+\epsilon)r)$ that will collide in a bucket with $q$ is $M=4=O(1)$.
\end{itemize}
\end{lemma}


\subsubsection{Index}

We construct $m = \frac{3}{\log(4/3)} \log n$ copies of the index (choosing $k = O(\log n)$ and $\tau = O(n^{1/\rho})$) above, denoted as $\mathbb{I}_1, \mathbb{I}_2, \cdots, \mathbb{I}_m$. Note that each index $\mathbb{I}_j$ has $2^k \cdot \tau$ buckets. An important property on this set of indexes is stated by the following Lemma, and its proof is given in Appendix~\ref{appendix:lsh-proof}.  

\begin{lemma}
    \label{lem:non-uniform-property_2}
    With probability at least $1-1/n$, for any pair of points $(a, b) \in A\times B$ with $\dist(a,b) \le r$, there exists an index $\mathbb{I}_j$ such that 
    \begin{itemize}
        \item $a,b$ will collide in some bucket of $\mathbb{I}_j$;
        \item The number of points in $A(a, (1+\epsilon)r)$ as well as $B(a, (1+\epsilon)r)$ colliding with $a$ is $M=O(1)$;
        \item The number of points in $A(b, (1+\epsilon)r)$ as well as $B(b, (1+\epsilon)r)$ colliding with $b$ is $M=O(1)$;
    \end{itemize}
\end{lemma}
\begin{proof}
    Consider any pair of points $(a, b) \in A \times B$ with $\lVert a -b\rVert \le r$ and an arbitrary index constructed as described above. From Lemma~\ref{lem:nnq}, with probability at least $1/4$ there exists a bucket in the index that contains both $a, b$ and the number of collisions of both $a$ and $b$ (with the rest of the points in $A\cup B$) is bounded by $O(1)$. 
    
    Let $F_j$ be the event that is true if there is a bucket in $\mathbb{I}_j$ that witnesses the collision of $a, b$ and the number of collisions of both $a, b$ is bounded by $O(1)$. Since $F_i, F_j$ are independent for $i\neq j$, we have $\Pr[\bar{F}_1 \cap \ldots \cap \bar{F}_C]=\Pr[\bar{F}_1]\cdot \ldots \cdot \Pr[\bar{F}_C] \leq (3/4)^{\frac{3}{\log(4/3)}\log n}\leq 1/n^3$. Let $Z$ be the number of pairs with distance at most $r$. We have $Z\leq n^2$. Let $G_i$ be the event which is true if for the $j$-th pair of points $a', b'$ with distance at most $r$, there is at least a copy of the index such that there exists a bucket that contains both $a', b'$ and the number of collisions of both $a, b$ is bounded by $O(1)$. Then $\Pr[G_1 \cap \ldots \cap G_Z]=1-\Pr[\bar{G}_1\cup \ldots \cup \bar{G}_Z]\geq 1-\Pr[\bar{G}_1]-\ldots-\Pr[\bar{G}_Z]\geq 1-n^2/n^3\geq 1-1/n$. Hence, with high probability, for any pair $a\in A, b\in B$ with distance at most $r$ there will be at least one bucket in the index such that, both $a, b$ are contained in the bucket and the number of collisions of both $a, b$ in the bucket is bounded by $M=O(1)$.
\end{proof}

In plain language, for each join result $(a,b)$, there exists at least one bucket such that $a,b$ will collide and the number of ``noisy'' points (with distance more than $(1+\epsilon)r$ from $a$ or $b$) inside this bucket is also bounded by $O(1)$, since points inside each bucket must be distinct. For simplicity, we denote such a bucket described by Lemma~\ref{lem:non-uniform-property}
as {\em proxy bucket} for the join result $(a,b)$. Later, we will see in the enumeration phase that each join result is only reported by one of its proxy bucket, thus guarantee the completeness of query results. However, an inherent challenges of duplication remains, i.e., de-duplication is necessary if a pair of points has more than one proxy buckets.


\stavros{If we run the current algorithm we have but instead of checking $O(n^\rho)$ points in a bucket when we insert a point or $O(n^{2\rho})$ points in bucket when we delete a point we can just check $O(1)$ points. Hence we would have the next result.}


\begin{theorem}
\label{the:high-non-uniform_2}
Let $A$ and $B$ be two sets of points in the hamming space $\mathbb{H}^d$, where $|A|+B|=n$, and let $\eps > 2, r$ be positive parameters. For $\rho=1/(1+\eps)$,
an index of $\O(dn+n^{1+\rho})$ space can be constructed in $\O(dn^{1+\rho})$ time such that all pairs of points within distance $r$ will be reported (with high probability) along with some pairs of points within distance $2(1+\eps)r$, with $\O(dn^{\rho})$ delay. The index can be updated in $\O(dn^{\rho})$ amortized time.
\end{theorem} 








====================================================

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\stavros{The next is a try to also improve the $2(1+\eps)$ approximation factor. After arguing as before and having proved Lemma~\ref{lem:non-uniform-property_2} we can continue as follows before we describe the algorithm.}

\newcommand{\Expec}{\mathbf{E}}
\begin{lemma}
Let $p\in P$ be a point in $\mathbb{H}^d$ and let $P(p, (1+\eps)r)$ be the points in $P$ with distance more than $(1+\eps)r$ from $p$. With probability at least $3/4$ the number of points in $P(p,(1+\eps)r)$ that will collide in every bucket with $p$ is $2\log (4\tau) + 1=O(\log n)$.
\end{lemma}
\begin{proof}
Let $h$ be one of the $\tau$ hash functions and let $q\in P(p,(1+\eps)r)$. From~\cite{} we have that $\Pr[h(p)=h(q)]\leq 1/n$.
Let $X(q)$ be a random variable which is $1$ if $h(p)=h(q)$, and $0$, otherwise.
Let $X=\sum_{q\in P(p, (1+\eps)r)}X(q)$. We have $\mu=\Expec[X]\leq 1$.
We have $\Pr[X\geq 2\log (4\tau) +1]\leq \Pr[X\geq (1+\frac{2\log (4\tau)}{\mu})\mu]$.
From Chernoff inequality\footnote{We use the version of Chernoff inequality where $\Pr[X\geq (1+\delta)\mu]\leq e^{-\delta^2\mu/(2+\delta)}$, for $\delta\geq 0$} we have
$\Pr[X\geq (1+\frac{2\log (4\tau)}{\mu})\mu]\leq e^{-\frac{2^2\log^2 (4\tau)/\mu}{2+2\log (4\tau)/\mu}}$.
Notice that $2+2\log (4\tau)/\mu\leq 4\log (4\tau) /\mu$, so 
$\Pr[X\geq 2\log (4\tau)+1]\leq e^{-\frac{\log^2 (4\tau)/\mu}{\log (4\tau)/\mu}}=e^{-\log (4\tau)} = \frac{1}{4\tau}$.

Let $G_i$ be the event which is true if point $p$ has at most $2\log (4\tau) + 1$ conflicts with points in $P(p,(1+\eps)r)$ at hash function $h_i$.
$\Pr[\cap_{i=1}^{\tau G_i]=1-\Pr[\bigcup_{i=1}^{\tau}\bar{G}_i]\geq 1-\frac{\tau}{4\tau}=3/4$.
\end{proof}




Let  $p$ be a point in $P$ and $P(p, (1+\epsilon)r)$ be the set of points in $P$ with distance more than $(1+\eps)r$ from $p$. Let $h$ be one hush function and let $q\in P(p,(1+\eps)r)$. From \cite{} we have that $\Pr[h(p)=h(q)]=\beta^k\leq \frac{1}{n}$.
Let $X(q)$ be a random variable which is $1$ if $h(p)=h(q)$, and $0$, otherwise.
Let $X=\sum_{q\in P(p, (1+\eps)r)}X(q)$. We have $\mu=E[X]\leq 1$.
Let $c$ be a constant we will decide later.
We have $\Pr[X\geq c\log n+1]\leq \Pr[X\geq (1+\frac{c\log n}{\mu})\mu]$.
From Chernoff inequality we have
$\Pr[X\geq (1+\frac{c\log n}{\mu})\mu]\leq e^{-\frac{c^2\log^2 (n)/\mu}{2+c\log (n)/\mu}}$.
Notice that $2+c\log (n)/\mu\leq 2c\log (n) /\mu$, so 
$\Pr[X\geq c\log n+1]\leq e^{-\frac{c\log^2 (n)/\mu}{2\log (n)/\mu}}=e^{-\frac{c}{2}\log n} = \frac{1}{n^{c/2}}$.

Hence with probability at least $1-\frac{1}{n^{c/2}}$, point $p$ will have at most $O(\log n)$ conflicts with points in $P(p, (1+\eps)r)$ in one hash function $h$.

Let $G_i$ be the event which is true if point $p$ has $O(\log n)$ conflicts with points in $P(p,(1+\eps)r)$ at hash function $h_i$.
$\Pr[\cap_{i=1}^{n^{\rho+1}} G_i]=1-\Pr[\bigcup_{i=1}^{n^{\rho+1}}\bar{G}_i]\geq 1-\frac{1}{n^{c/2-\rho-1}}$.
(The number of buckets we construct in Lemma~\ref{lem:non-uniform-property_2} is $O(n^{\rho}\log n)$ which is also bounded (for simplicity) by $n^{\rho+1}$ in the bound above).

Let $F_i$ be the event which is true if point $p_i\in P$ has  $O(\log n)$ conflicts in all the $O(n^{\rho}\log n)$ hash functions.
$\Pr[\cap_{i=1}^{n} F_i]=1-\Pr[\bigcup_{i=1}^{n}\bar{F}_i]\geq 1-\frac{1}{n^{c/2-\rho-2}}$.

If we set $c=2(\rho +3)\leq 8$ then with probability at least $1-1/n$ every point $p\in P$ will have at most $8\log n$ conflicts with $P(p, (1+\eps)r)$ in every hash function /bucket.

\stavros{The we could use this result in several ways. For example, when we insert a point $a$ in a bucket $\square$ we could argue that we check all points in $B_\square$ until we find a point within distance $r$ or until there are no points within distance $r$. Notice that according to our proven argument this procedure will take $O(\log n)$ time (in one bucket) with high probability. Similarly, we can argue for deletions. In that way we can say that with high probability the delay/update is $O(dn^{\rho})$ and we report all pairs within distance $r$ with high probability and might report pairs with distance $(1+\eps)r$. (notice that now we have a better approximation error and complexities but the complexities hold with high probability, which was not the case before. Of we want to argue that the delay/update is not randomized then we can stop the procedure after checking more than $O(\log n)$ elements in $B_\square$ when we insert a new point $a$ in a bucket $\square$ (similarly for deletion). Since we have argued that with high probability it is not possible to have more than $O(\log n)$ conflict of a point in a bucket then with high probability we will report anything the delay/update will be deterministic and the error will be $(1+\eps)$.}





==> lsh_new2.tex <==
\clearpage
\newpage
\newcommand{\Expec}{\mathbf{E}}
\begin{lemma}
\label{lemma:prob}
Let $p\in P$ be a point in $\mathbb{H}^d$ and let $P(p, (1+\eps)r)$ be the points in $P$ with distance more than $(1+\eps)r$ from $p$. With probability at least $3/4$ the number of points in $P(p,(1+\eps)r)$ that will collide in any bucket with $p$ is $2\log (4\tau) + 1=O(\log n)$.
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lemma:prob}]
Let $h$ be one of the $\tau$ hash functions and let $q\in P(p,(1+\eps)r)$. From~\cite{} we have that $\Pr[h(p)=h(q)]\leq 1/n$.
Let $X(q)$ be a random variable which is $1$ if $h(p)=h(q)$, and $0$, otherwise.
Let $X=\sum_{q\in P(p, (1+\eps)r)}X(q)$. We have $\mu=\Expec[X]\leq 1$.
We have $\Pr[X\geq 2\log (4\tau) +1]\leq \Pr[X\geq (1+\frac{2\log (4\tau)}{\mu})\mu]$.
From Chernoff inequality\footnote{We use the version of Chernoff inequality where $\Pr[X\geq (1+\delta)\mu]\leq e^{-\delta^2\mu/(2+\delta)}$, for $\delta\geq 0$} we have
$\Pr[X\geq (1+\frac{2\log (4\tau)}{\mu})\mu]\leq e^{-\frac{2^2\log^2 (4\tau)/\mu}{2+2\log (4\tau)/\mu}}$.
Notice that $2+2\log (4\tau)/\mu\leq 4\log (4\tau) /\mu$, so 
$\Pr[X\geq 2\log (4\tau)+1]\leq e^{-\frac{\log^2 (4\tau)/\mu}{\log (4\tau)/\mu}}=e^{-\log (4\tau)} = \frac{1}{4\tau}$.

Let $G_i$ be the event which is true if point $p$ has at most $2\log (4\tau) + 1$ conflicts with points in $P(p,(1+\eps)r)$ at hash function $h_i$.
$\Pr[\cap_{i=1}^{\tau} G_i]=1-\Pr[\bigcup_{i=1}^{\tau}\bar{G}_i]\geq 1-\frac{\tau}{4\tau}=3/4$.
\end{proof}

Hence, from Lemma~\ref{lemma:prob} and \cite{} we have the next lemma.
\begin{lemma}[\cite{gionis1999similarity_2}]
\label{lem:nnq_2}
    For a set of $n$ points $P$ in hamming space $\mathbb{H}^d$ and a distance threshold $r$, by choosing $k=O(\log n)$, and $\tau=O(n^{\rho})$, the following two properties hold for every point $q \in P$:
\begin{itemize}
    \item Let $p$ be a point such that $\dist(p, q) \leq r$. With probability at least $3/4$, the point $q$ will collide in some bucket with point $p$;
    \item Let $P(q, (1+\epsilon)r)$ be the set of points in $P$ with distance more than $(1+ \epsilon)r$ from $q$. With probability at least $3/4$, the total number of distinct points in $P(q, (1+\epsilon)r)$ that will collide in any bucket with $q$ is $O(\log n)$.
\end{itemize}
\end{lemma}



==> prelim.tex <==
\section{Preliminaries}
\label{sec:prelim}
%In this section, we introduce a few useful tools including data structures for range searching and known techniques for transforming a static data structure to a dynamic one.

%\subsection{Range search data structures}

%\mparagraph{Range tree}
%A range tree~\cite{bentley1978decomposable} on a set $P$ of $n$ points in $\Re$ is a balanced binary search tree of $O(\log n)$ height. The points are stored in the leaves of the tree while each internal node $v$ stores the smallest and the largest value, $x_v^-, x_v^+$, respectively contained in its subtree.
%The node $v$ is associated with an interval $I_v=[x_v^-, x_v^+]$ and the subset $P_v=I_v\cap P$.
%A $d$-dimensional range tree $\T$ on a set $P$ of points in $\Re^d$ is a recursively defined $d$-level balanced binary search tree.
%See~\cite{de1997computational} for details.
%\begin{figure}
%\centering
%  \minipage{0.5\textwidth}
%  \centering
%  \includegraphics[width=0.57\linewidth]{DynamicEnumerationNEW/pods2021/range-tree.pdf}
%  \caption{An illustration of range tree.}
%  \label{fig:range-tree}
%  \endminipage\hfill
%  \minipage{0.5\textwidth}
%  \centering
%  \includegraphics[width=0.75\linewidth]{DynamicEnumerationNEW/pods2021/wspd.pdf}
%    \caption{Well-separated pair in the WSPD.}
%    \label{fig:wspd}
%\endminipage\hfill
   % \includegraphics[scale=0.6]{DynamicEnumerationNEW/pods2021/range-tree.pdf}
  %  \caption{An illustration of range tree $\T$ in $\Re^3$.}
 %   \label{fig:range-tree}
%\end{figure}
%For each node $u$ of the $d$-th level of $\T$, we associate a $d$-tuple of $\T$ $\pi(u)=\langle u_1, u_2, \ldots, u_d=u\rangle$, where $u_i$ is the node at the $i$-th level of $\T$ to which the level-$d$ subtree of $\T$ containing $u_i$ is connected.
%We associate the rectangle $\square_u=\prod_{j=1}^d I_{u_j}$ with the node $u$.
%For a rectangle $b=\prod_{i=1}^d [b_i^-, b_i^+]$, a $d$-level node is called a \emph{canonical node} if for every $i=1,\ldots, d$, $I_{u_i}\subseteq [b_i^-, b_i^+]$ and $I_{p(u_i)}\not\subseteq [b_i^-, b_i^+]$, where $\pi(u)=\langle u_1,\ldots, u_d=u\rangle$ and $p(u_i)$ is the parent of node $u_i$ in the level-$i$ tree rooted at $u_{i-1}$.
%For any rectangle $b$, there are $O(\log^d n)$ canonical nodes in $\T$, which can be computed in $O(\log^d n)$ time.


\mparagraph{Quadtree}
A $d$-dimensional quadtree~\cite{har2011geometric, samet1989spatial} over a point set $P$ is a tree data structure in which each node $u$ is associated with a box $\square_u$ in $\Re^d$ and each internal node has exactly $2^d$ children. It recursively subdivides the space into $2^d$ equal size boxes until a box contains at most one point from $P$.
Let $\mathcal{S}=\frac{\max_{x,y\in P}\lVert x-y \rVert_2}{\min_{x,y\in P}\lVert x-y \rVert_2}$ be the \emph{spread} of $P$. $\T$ can be constructed in $O(n\log \mathcal{S})$ time, it has $O(n\log\mathcal{S})$ space, and $O(\log\mathcal{S})$ height. %See~\cite{har2011geometric} for details on quadtrees.
%Given a sphere $\mathcal{B}$, the quadtree can be used to find $O(\log \mathcal{S} + \eps^{d-1})$ nodes such that the union of their regions completely covers $\mathcal{B}\cap P$ and might cover some parts of $(1+\eps)\mathcal{B}$.

\mparagraph{Well Separated Pair Decomposition (WSPD) \cite{callahan1995decomposition, har2006fast, har2011geometric}} %WSPD can be built on a quadtree for storing input points $P$. 
%
%
%For a set of points $P$, let $\diam(P) = \max_{x,y\in P} \lVert x-y\rVert_2$. For two sets of points $P_1,P_2$, let $\dist(P_1, P_2) = \min_{x \in P_1, y\in P_2} \lVert x -y\rVert_2$. 
%
%\begin{definition}[Well-separated Pair Decomposition]
%\label{def:wspd}
%The WSPD is defined as follows.  
Given a set $P$ of $n$ points in $\mathbb{R}^d$ and a parameter $0< \eps < \frac{1}{2}$, a set of $s$ pairs $W=\{(X_1, Y_1), (X_2, Y_2), \cdots, (X_s, Y_s)\}$ is an $\eps$-WSPD if the following conditions hold: (1) for any $i \in \{1,2,\cdots,s\}$, $X_i, Y_i \subseteq P$ and $X_i\cap Y_i=\emptyset$; (2) for each pair of points $x, y \in P$, there exists a unique pair $(X_j, Y_j)\in W$ such that $x \in X_j$ and $y\in Y_j$; (3) $s=O(\eps^{-d}n)$ and (4) for any $i \in \{1,2,\cdots,s\}$, $\max\{\diam(X_i), \diam(Y_i)\} \leq \eps \cdot \dist(X_i, Y_i)$, where $\diam(P) = \max_{x,y\in P} \lVert x-y\rVert_2$ and $\dist(P_1, P_2) = \min_{x \in P_1, y\in P_2} \lVert x -y\rVert_2$. 
%\end{definition}
%Each pair $(X_i, Y_i)$ is {\em well-separated} in the sense that any two points across $X_i, Y_i$ have their distance being at least $\frac{1}{\eps}$-factor of the largest distance between points inside $X_i$ or $Y_i$. %see Figure~\ref{fig:wspd}.
%\begin{figure}[t]
%    \centering
%    \includegraphics[scale=0.7]{DynamicEnumerationNEW/pods2021/wspd.pdf}
%    \caption{An illustration of well-separated pair in the WSPD.}
%    \label{fig:wspd}
%\end{figure}
In~\cite{har2011geometric, har2006fast}, a compressed (compressed) quadtree is used to construct an $\eps$-WSPD efficiently.
In particular, an $\eps$-WSPD $W$ can be constructed in $O(n\log n +\eps^{-d}n)$ time such that each pair $(X_i, Y_i)\in W$ is a pair of nodes in a quadtree over the points set of points $P$.
%The sets of points corresponding to $X_i, Y_i$ are denoted as $P \cap \square_{X_i}, P \cap \square_{Y_i}$ respectively.
It is also known that for each pair $(X_i, Y_i) \in W$, (i) $\square_{X_i}\cap \square_{Y_i}=\emptyset$, and (ii) $\max\{\diam(\square_{X_i}), \diam(\square_{Y_i})\}\leq \eps \dist(\square_{X_i}, \square_{Y_i})$. %Another important property that will be frequently used on $W$ and $\T$ is stated as below.
Furthermore, given a set $P$ of $n$ points with $O(\poly(n))$ spread its WSPD $W$ built on a quadtree $\T$, $\T$ has height $\O(1)$ and every node in $\T$ participates in $\O(\eps^{-d})$ pairs of $W$ (see~\cite{har2011geometric} for details).
%\begin{lemma}[\cite{har2011geometric}]
%\label{lem:propQuad}
%Given a set $P$ of $n$ points with $O(\poly(n))$ spread and its WSPD $W$ built on a quadtree $\T$, $\T$ has height $\O(1)$ and every node in $\T$ participates in $\O(\eps^{-d})$ pairs of $W$.
%\end{lemma}

 %We assume that $\eps$ is a small constant, so the complexity dependency on $\eps$ is hidden in $O(.)$.

%\paragraph{BBD tree.}
%A balanced box decomposition (or BBD for short) tree~\cite{arya2000approximate, arya1998optimal} is a variant of the \emph{quadtree}~\cite{har2011geometric, samet1989spatial}. A BBD tree $\T$ on a set $P$ of $n$ points in $\mathbb{R}^d$, is a balanced binary tree of size $O(n)$ and height $O(\log n)$ with $n$ leaves. It can be constructed in $O(n\log n)$ time.
%Every box has a bounded aspect ratio and every $2d$ levels of descent in the tree, the size of the associated cells decreased by at least a factor of $1/2$, where the size of a cell is defined as the length of its longest side.
%Each node is associated with a box in $\mathbb{R}^d$ or the set theoretic difference of two nested boxes $\square_v^O, \square_v^I$ (rectangular annulus) with $\square_v^I$ possibly being empty. Hence each box $v$ is associated with an annular region $\square_v=\square_v^O\setminus \square_v^I$.


%Given a sphere $B$ of radius $1$, the BBD tree in \cite{arya2000approximate, arya1998optimal}
%returns $O(\log n + \eps^{d-1})$ nodes
%such that the union of their regions
%completely covers $B\cap P$ and might cover some parts of $(1+\eps)B$.
%Given $x\in \Re^d, r\geq 0, \eps>0$, the BBD tree $\T$ can be %used to answer an $\eps$-approximate neighborhood query:
%    \begin{itemize}
%        \item all points of $P$ within distance $r$ from $x$ will be returned;
%        \item no point of $P$ farther than $(1+\epsilon)r$ from $x$ will be returned;
%    \end{itemize}
%Points that are at distance from $x$ between $r$ and $(1+\eps)r$ from $x$ may or may not be reported. The time complexity of such a query is $O(\log n + \eps^{1-d}+k)$, where $k$ is the output size. 

%In~\cite{eppstein2005skip, mount2010dynamic}, the dynamic version of BBD tree was proposed, with $\O(1)$ time for maintenance under per update.



%\mparagraph{Dynamization techniques}
%The following is the standard technique proposed by Bentley and Saxe~\cite{bentley1980decomposable} (see also \cite{erickson2011static}) for transforming a static data structure to a dynamic one, for any decomposable query.
%To build a data structure on a set $X$ of $n$ objects that can be updated efficiently under updates, the idea is to partition $X$ into $m=\ceiling{\log_2 n}$ groups $L_0 , \ldots, L_{m-1}$, such that (1) $L_i\subseteq X$; (2) $L_i\cap L_j=\emptyset$; (3) $\bigcup_{i=1,\ldots, m-1} L_i=X$; (4) $|L_i| = 0$ or $|L_i| = 2^i$.
%A static data structure $\T_i$ is built for each group $L_i$.
%Let $P(x), T(x)$ be the construction time and the query time of such a static data structure $\T_i$ that contains $x$ elements.
%In order to answer a query over the new data structure, we visit each non-empty group $L_i$, run the query procedure over the static data structure $\T_i$ and return their unions.
%The total query time is $\sum_{i=0}^{m-1} T(2^i) <m \cdot T(n) =O(T(n)\log n)$. 
%When a new object $x$ is inserted, let $i$ be the smallest data structure such that $L_i = \emptyset$. Set $L_i = \{x\} \cup \bigcup_{j <i} L_j$. We delete all previous static data structures in $L_0,\ldots, L_{i-1}$, and construct a new static data structure $\T_i$ for $L_i$.
%By charging $\sum_{i=0}^{\log n}\frac{P(2^i)}{2^i}$ to each insertion, the amortized time is $O(\frac{P(n)}{n} \log n)$. 
%When an object is deleted, we perform \emph{weak deletion}: delete it from the static data structure $\T_i$ containing it, without changing the structure of $\T_i$. 
%When more than half number of objects are deleted, we just rebuild everything from scratch. The amortized cost of a deletion is $O(\frac{P(n)}{n} + D(n))$, where $D(\cdot)$ is the time to perform a weak deletion.

==> wspd.tex <==
\subsection{Variable Similarity Threshold}
\label{sec:wspd}

We now describe the data structure when the threshold $r$ is not fixed but instead specified as part of the query. We assume that the spread of $A\cup B$ is polynomially bounded, i.e., $sp(A\cup B)=\frac{\max_{p,q \in A\cup B}\dist(p,q)}{\min_{p,q\in A\cup B}\dist(p,q)}=n^{O(1)}$. We use quad tree and well-separated pair decomposition (WSPD) for our data structure. We describe them briefly here and refer the reader to~\cite{har2011geometric}.

\paragraph{Quad tree and WSPD.}
A $d$-dimensional quad tree~\cite{har2011geometric, samet1989spatial} over a point set $P$ is a tree data structure $\T$ in which each node $u$ is associated with a hypercube $\square_u$ in $\Re^d$ and each internal node has exactly $2^d$ children.
The root is associated with a hypercube containing $P$. For a node $u$, let $P_u=P\cap \square_u$. A node $u$ is a leaf if $|P_u|\leq 1$.
The tree recursively subdivides the space into $2^d$ congruent hypercubes until a box contains at most one point from $P$.
If $sp(P)=n^{O(1)}$, the height of $\T$ is $O(\log n)$.

Given two point sets $A, B\subset \Re^d$, with $|A|+|B|=n$,
and a parameter $0< \eps < \frac{1}{2}$, a family of pairs $\W=\{(A_1, B_1), (A_2, B_2), \cdots, (A_s, B_s)\}$ is an $\eps$-WSPD if the following conditions hold: (1) for any $i\leq s$, $A_i\subseteq A$, $B_i\subseteq B$ (2) for each pair of points $(a,b) \in A\times B$, there exists a unique pair $(A_j, B_j)\in \W$ such that $a \in A_j$ and $b\in B_j$ (3) for any $i\leq s$, $\max\{\diam(A_i), \diam(B_i)\} \leq \eps \cdot \dist(A_i, B_i)$, where $\diam(X) = \max_{x,y\in X} \dist(x,y)$ and $\dist(X, Y) = \min_{x \in X, y\in Y} \dist(x,y)$ (see Figure~\ref{fig:wspd}). 
As shown in~\cite{har2011geometric, har2006fast} if $sp(A\cup B)=n^{O(1)}$, a quad tree $T$ on $A\cup B$ can be used to construct, in time $O(n\log n + \eps^{-d}n)$, a WSPD $\W$ of size $O(\eps^{-d}n)$ such that
each pair $(A_i, B_i)\in \W$ is associated with pair of nodes $(\square_i, \boxplus_i)$ in $\T$ where $A_i=A\cap \square_i$ and $B_i=B\cap \boxplus_i$.
It is also known that for each pair $(A_i, B_i)\in \W$ (i) $\square_i\cap \boxplus_i=\emptyset$, and (ii)
$\max\{\diam(\square_i), \diam(\boxplus_i)\}\leq \eps\dist(\square_i, \boxplus_i)$ (see Figure~\ref{fig:wspd}).
We will use $\W=\{(\square_1,\boxplus_i), \ldots, (\square_s,\boxplus_s)\}$ to denote the WSPD, with $A_i, B_i$ being implicitly defined from their nodes.
%\footnote{In fact, the algorithm described in~\cite{har2011geometric} works even if $sp(A\cup B)$ is unbounded but one has to use a compressed quad tree instead of a regular quad tree.}
Using the techniques in~\cite{callahan1995dealing, fischer2005dynamic}, the quad tree $\T$ and the WSPD $\W$ can be maintained under insertions and deletions of points in $\O(\eps^{-d})$ time.
 
 
\paragraph{Data structure.} 
We construct a quad tree $\T$ on $A\cup B$.
For each node $u \in \T$, we store a pointer $A_u$ (and $B_u$) to the leftmost leaf of subtree $\T_u$ that contains a point from $A$ (and $B$). Furthermore, we store a sorted list $A_{\T}$ (and $B_{\T}$)of the leaves that contain points from $A$ (and $B$). We use these pointers and lists to report points in $\square_u$ with $O(1)$ delay.
Using $\T$, we can construct a WSPD $\W=\{(\square_1, \boxplus_1),\ldots, (\square_s, \boxplus_s)\}$, $s=O(\eps^{-d})$.
%The tripartite graph $G = (A \cup C \cup B, E_1 \cup E_2)$ is defined as follows. Set $C = \{C_1, \ldots, C_s\}$.
%For each $i\leq s$, $(a,c)\in E_1$ for all $a\in A_i$ and $(c,b)\in E_2$ for all $b\in B$. Again, we do not maintain $E_1$ and $E_2$ explicitly. They are defined implicitly by $\square_i, \boxplus_i$.
For each $i$, let $\Delta_i=\min_{p\in \square_i, q\in\boxplus_i}\dist(p,q)$. We store all pairs $(\square_i, \boxplus_i)$ in a red-black tree $\mathcal{Z}$ using $\Delta_i$ as the key. 
The data structure has $O(\eps^{-d}n)$ space and $O(\eps^{-d}n\log n)$ construction time.
%The size of the data structure is $O(\eps^{-d}n)$ and it can be constructed in $O(\eps^{-d}n\log n)$ time.


\paragraph{Update.} After inserting or deleting an input point, the quad tree $\T$ and $W$ can be updated in $\O(\eps^{-d})$ time, following the standard techniques in ~\cite{callahan1995dealing, fischer2005dynamic}. As there are at most $\O(\eps^{-d})$ pairs changed, we can update $\mathcal{Z}$ in $\O(\eps^{-d})$ time. Furthermore, we note that there are only $O(1)$ changes in the structure of quad tree $\T$ and the height of $\T$ is $O(\log n)$, so we can update all necessary pointers $A_u, B_u$ and sorted lists $A_{\T}, B_{\T}$ in $O(\log n)$ time.

%Note that the $\eps$-WSPD can be maintained under updates in $\O(1)$ time \cite{callahan1995dealing, fischer2005dynamic}.

%Next, we will explain how to update $\C$. Without loss of generality, assume the update is from $A$, say $a$. 

%Let $W_1, W_2$ be the set of pairs deleted from and inserted to $W$ respectively. For each pair $(X_i,Y_i)\in W_1$, if $(X_i, Y_i) \in \C$, we remove it from $\C$. For each pair $(X_i, Y_i)\in W_2$, we first check whether it is active. If yes, we compute $\dist(\square_{X_i}, \square_{Y_i})$ and insert this pair to $\C$.

%It remains to check whether an old pair of $W$ should be updated from $\C$, after the update of $a$. Without loss of generality, assume $a$ is inserted (the deletion can be handled symmetrically). Let $u \in T$ be the new leaf node containing $a$. Consider each node $v$ lying on the path from the root to $u$. For each pair including $v$ in $W$, say $(v,t)$, if $(v,t) \notin \C$, we check whether $(v,t)$ turns active after inserting $a$. If yes, we compute the value of $\dist(\square_v, \square_t)$ and insert it in $\C$. The update time is $\O(\eps^{-d})$; the detailed proof is given in Appendix~\ref{appendix:wspd}.


\paragraph{Enumeration.}
We traverse $\mathcal{Z}$ in order until we reach a pair $(\square_j, \boxplus_j)$ with $\Delta_j>r$.
For each pair $(\square_i, \boxplus_i)$ we traverse we enumerate $(a,b)\in (A\cap \square_i) \times (B\cap \boxplus_i)$ using the stored pointers and the sorted lists $A_\T, B_\T$.
The delay guarantee is $O(1)$.
%All enumerated pairs form an $(1+\eps)$-approximation of the join result.
%The proof of correctness is provided in the Appendix~\ref{appendix:wspd}.


%It suffices to show that every pair of points within distance $r$ must be reported, while any pair of points with distance larger than $(1+\eps)r$ will not be reported.
Let $(a, b) \in A \times B$ be a pair with $\dist(a,b)\leq r$. Implied by the definition, there exists a unique pair $(A_i, B_i)\in \W$ such that $a\in A_i$ and $b\in B_i$. Notice that  $\dist(\square_i, \boxplus_i) \leq\dist(a,b) \leq r$. Thus, all join results across $A_i, B_i$ will be reported, including $(a,b)$.  Next, let $(A_i, B_i)$ be a pair that is found by the enumeration procedure in $\mathcal{Z}$, with $\dist(\square_i, \boxplus_i)\leq r$.
For any pair of points $x \in \square_i, y \in \boxplus_i$, we have
%their distance can be bounded as
$\dist(x,y) \le & \dist(\square_i,\boxplus_i)+\diam(\square_i)+\diam(\boxplus_i) 
\le  (1+2\cdot \frac{\eps}{2}) \cdot \dist(\square_i,\boxplus_i) \le (1+\eps)r$,
thus any pair of points with distance strictly larger than $(1+\eps)r$ will not be reported.


\begin{theorem}
Let $A, B$ be two sets of points in $\mathbb{R}^d$ for constant $d$, with $O(\poly(n))$ spread and $|A| + |B| = n$.
A data structure of $O(\eps^{-d}n)$ space can be built in $\O(\eps^{-d}n)$ time and updated in $\O(\eps^{-d})$ time, while supporting $\eps$-approximate enumeration for similarity join under any $\ell_p$ metric with $O(1)$ delay, for any query similarity threshold $r$.
\end{theorem}

